WFA-IRL: Inverse Reinforcement Learning of Autonomous Behaviors Encoded as Weighted Finite Automata

This paper presents a method for learning logical task specifications and cost functions from demonstrations. Constructing specifications by hand is challenging for complex objectives and constraints in autonomous systems. Instead, we consider demonstrated task executions, whose logic structure and transition costs need to be inferred by an autonomous agent. We employ a spectral learning approach to extract a weighted finite automaton (WFA), approximating the unknown task logic. Thereafter, we define a product between the WFA for high-level task guidance and a labeled Markov decision process for low-level control. An inverse reinforcement learning (IRL) problem is considered to learn a cost function by backpropagating the loss between agent and expert behaviors through the planning algorithm. Our proposed model, termed WFA-IRL, is capable of generalizing the execution of the inferred task specification in a suite of MiniGrid environments.

==> tex/Experiments_old.tex <==
\section{Evaluation}
\label{sec:experiments}

We demonstrate our model's ability to infer task structure and transition costs from demonstration with the DoorKey task introduced in Fig~\ref{fig:doorkey}. 

%to learn the task structure, as well as the cost function with a DoorKey task in a simulated Minigrid environment \cite{gym_minigrid} (see Fig~\ref{fig:doorkey}).

\subsection{Minigrid environment}
% Environment configurations
We simulated the DoorKey task in an $8 \times 8$ Minigrid environment \cite{gym_minigrid}. Each grid cell can have a semantic category among $Wall$, $Key$, $Door$ or $Empty$. A new grid configuration is randomly generated at each episode with a vertical wall (in gray) at a random column, dividing the grid into left and right rooms. The two rooms are connected via a door (in yellow) at the column of the wall but at a random row. The agent (red arrow) and a key (in yellow) are spawned at random locations in the left room while the goal (in green) is at the bottom right corner of the right room. There is a $30\%$ chance that the door is open so the agent may proceed to the goal directly and ignore the key. Otherwise, the agent should first pick up the key to unlock the door and then reach the goal. The state $\bfx_t$ at time $t$ includes the grid configuration $\bfm_t \in \crl{Wall, Key, Door, Empty}^{8 \times 8}$, the agent position $\bfp_t \in \crl{1,\ldots,8}^2$, the agent direction $d_t \in \crl{Up, Left, Down, Right}$, and an object that the agent is carrying $o_t \in \crl{Key, Empty}$. The control space $\calU$ is defined as turn left, turn right, move forward, pick up an object, drop an object, and toggle an object (e.g., open or close a door).

%The task specifications are expressed as a linear temporal logic (LTL) formula \cite{Baier2008Principles}. Definition and semantics of an LTL formula can be found in Appendix.~\ref{sec:ltl}. An agent can either pick up the key ($p_1$) if the door is locked or go through the door directly if it is open ($p_2$), and finally reach the goal ($p_3$). Then the true LTL formula of the DoorKey task is 
%\begin{equation}
%\label{eq:doorkey_ltl}
%\phi = \prl{\prl{\prl{\lnot p_2 \cup p_1} \wedge (\lozenge p_2)} \vee \prl{p_2 \wedge \lnot p_1}} \wedge \prl{\lozenge p_3}.
%\end{equation}


\subsection{Demonstrations}
We collect positive and negative demonstrations $\calD$ in \eqref{eq:demo_set} as follows. A shortest path algorithm with cost of $1$ for any feasible transition is used to collect $100$ trajectories with labels $s=1$, which reach the goal. Another $100$ trajectories with labels $s=0$, which do not reach the goal are collected using random exploration. All $200$ trajectories are used to learn a WFA representation of the task via the spectral method in Sec.~\ref{sec:spectral_method}. However, only the positive demonstrations with labels $s=1$ are used to learn the cost function $c$, as described in Sec.~\ref{sec:planning} and~\ref{sec:cost_learning}.


%use two policies to 


\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{fig/cost_function.png}
\caption{Neural network architecture representing the transition cost $c_\theta(\bfx_t, \bfu_t)$ of a state-control pair $\bfx_t, \bfu_t$. The state $\bfx_t$ consists of the grid image $\bfm_t$, the agent position $\bfp_t$, direction $d_t$, object it is carrying $o_t$. The grid $m_t$ is fed through a convolutional neural network (Conv), while the discrete variables $\bfp_t$, $d_t$, $o_t$ and the control $\bfu_t$ are converted to embedding vectors (Embed) to provide vector latent representations for learning the cost function. The concatenated vector of Conv and Embed layer outputs is passed through three fully-connected layers (Dense) to obtain $c_\theta(\bfx_t, \bfu_t)$. The numbers ``96'', ``64'', ``32'' and ``1'' indicate the sizes of the hidden vectors.}
\label{fig:cost_function}
\end{figure*}

\subsection{Neural network cost representation}
\label{sec:cost_representation}
%The state space $\calX$ of the Minigrid environment includes agent states (e.g., agent position $p_t$, agent direction $d_t$, and object that the agent is carrying $o_t$) and environment states (e.g. grid configuration $m_t$ including key location and door status). The control space $\calU$ is defined as turn left, turn right, move forward, pick up an object, drop an object, and toggle an object (e.g., open or close a door). 
We use a neural network, shown in Fig.~\ref{fig:cost_function} to learn a nonlinear cost function $c_\theta$, mapping from each state-control pair to a non-negative cost value. The grid is provided as a 3-channel image $\bfm_t$ where each channel represents the object, its color, and status (door open or closed). The grid image is passed through a convolutional neural network with 2 series of convolutional + ReLU + max-pooling layers. The first convolutional layer uses 32 channels, $3\times 3$ filter size, stride $1$, and padding $1$, while the second convolutional layer uses $64$ channels, $1\times1$ filter size, stride $1$ and padding $0$. The resulting image is flattened and passed through two fully-connected layers with $64$ and $32$ units and ReLU activations. To provide vector representations for downstream learning, we use embedding layers to convert an agent state and control to vectors of fixed size. The agent position $\bfp_t$, direction $d_t$, and object $o_t$ are converted to embeddings of size $16$, $8$, and $8$ respectively, and the control is converted to an embedding of size $32$. The vector representation of the grid image after convolution and the agent and control embeddings are concatenated and passed through three fully-connected layers of size $64$, $32$, and $1$ with ReLU activations. The neural network cost representation $c_\theta$ is trained in PyTorch \cite{Paszke2019Pytorch} with Adam optimizer \cite{Kingma2014ADAM}.


\subsection{Baseline comparison and metrics}
We compare our method with maximum entropy inverse reinforcement learning (MaxEnt IRL)~\cite{Ziebart2008MaxEnt}, which finds a maximum entropy policy whose expected state-control visitation frequency matches that of the demonstrations. Although we study a finite state space using the Minigrid environment, the number of possible states is very large as the grid map configurations are generated randomly. Thus, representing the cost as a linear function over state-control feature vectors in a tabular setting, as in \cite{Ziebart2008MaxEnt}, quickly becomes intractable. We instead use the same neural network cost representation described above to parameterize $c_\theta(\bfx, \bfu)$. MaxEnt IRL obtains a maximum entropy policy given a cost estimate $c_\theta$ via ``soft'' value iteration where the ``max'' operator in the Bellman backup is replaced by a ``log-sum-exponential'' operator. The MaxEnt IRL baseline does not have access to $h$ and is not approximating it from the demonstrations either. It only initializes its value function to be zero at states $\bfx$ such that the agent position $\bfp$ is at the goal.

During testing, we randomly generate another set of $100$ grid environments that are not seen in the training set. We evaluate the baseline and our method on two metrics: trajectory success rate (\textit{TSR}) and modified Hausdorff distance (\textit{MHD}). In the test set, the agent iteratively applies a control input at each state using its learned policy in \eqref{eq:boltzmann_agent_policy}. \textit{TSR} records the success rate of the resulting trajectories where success is defined as reaching the goal cell (green) within twice the number of steps of the shortest path trajectory. Among the successful trajectories, \textit{MHD} compares how close the agent trajectories $\bfx_{1:T_n,A}^n$ are to the expert trajectories $\bfx_{1:T_n,E}^n$:
\begin{align}
&\textit{MHD} (\crl{\bfx_{1:T_n,A}^n},\crl{\bfx_{1:T_n,E}^n}) = \\
& \;\;\frac{1}{N} \sum_{n=1}^N \max\biggl\{\frac{1}{T_n}\sum_{t=1}^{T_n} d(\bfx_{t,A}^n, \crl{\bfx_{1:T_n,E}^n}), \notag\\
&\qquad\qquad\qquad\frac{1}{T_n}\sum_{t=1}^{T_n} d(\bfx_{t,E}^n, \crl{\bfx_{1:T_n,A}^n}) \biggr\},\notag 
\end{align}
%
where $d(\bfx_{t,A}^n, \crl{\bfx_{1:T_n,E}^n})$ is the minimum Euclidean distance from the state $\bfx_{t,A}^n$ at time $t$ to any state in $\bfx_{1:T_n,E}^n$. This metric indicates whether a policy has learned different modes when the door is open versus locked. If a trajectory is successful but its \textit{MHD} is high, it suggests that the agent is taking a suboptimal trajectory, e.g., the agent is always looking for a key, even when the door is already open. 


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig/trajectories.png}
\caption{Example trajectories generated by our model during test time. The agent learns the desired behavior of ignoring the key when the door is open from demonstrations. In the first row, when the door is locked, the agent picks up the key to open the door. In the second row, the agent realizes that the door is open and thus ignores the key. In the third row, the agent first picks up the key but later drops it, causing extra steps to finish the task. This exceeds the required number of steps and is regarded as a failed case. Frames of picking up/ignoring the key and unlocking/walking through the door are shown while intermediate frames are omitted.}
\label{fig:trajectories}
\end{figure*}
% trajectories obtained with random seed 1, 3, 5

\subsection{Results}
% Learning with WFA
% that describes the LTL formula of the task
We use the Scikit-SpLearn toolbox \cite{Arrivault2017SpLearn} to learn the weighted finite automaton, representing $h_\psi$. The hyperparameters for the spectral learning method are the rank of the automaton and the size of the basis, which determines the size of the Hankel matrix that is estimated empirically from the demonstrations. We vary the maximum size of elements used for the Hankel matrix between 2 and 8 (these are parameters \texttt{lrows} and \texttt{lcolumns} in the toolbox) and the matrix \texttt{rank} between 2 to 10. The hyperparameter configuration (\texttt{lrows} = 4, \texttt{lcols} = 4, \texttt{rank}= 7) that achieves the lowest prediction loss is used.


\begin{table}
  \centering
  \caption{Test results from the Minigrid environment \cite{gym_minigrid} on the DoorKey task, including the trajectory success rate (\textit{TSR}) and modified Hausdorff distance (\textit{MHD}) between the agent and the expert trajectories.}
  \label{tb:test_results}
  \begin{tabular}{c c c}
    \toprule
    Model & \makecell{\textit{TSR} (\%)} & \makecell{\textit{MHD}} \\
    \midrule
    \texttt{MaxEnt IRL} & 67 & 1.383 \\
    \texttt{Ours} & \textbf{92} & \textbf{0.254} \\
    \bottomrule
  \end{tabular}
\end{table}

Table~\ref{tb:test_results} shows the performance of MaxEnt IRL and our method evaluated according to the \textit{TSR} and \textit{MHD} metrics. First, MaxEnt IRL does not solve the navigation task as successfully as our method does. \textit{TSR} for MaxEnt IRL is much lower at $67\%$ versus ours at $91\%$. Empirically, we find that the MaxEnt IRL agent sometimes does not pick up the key when the door is locked, showing that it fails to find the high-level logical dependence between a locked door and a key. We measure \textit{MHD} to quantify the difference between the successful trajectories of the agent and the expert. Our model has a much smaller difference with a low \textit{MHD}. On the other hand, MaxEnt IRL does not always find the shortest path to the key subgoal. It sometimes wanders around in the left room without knowing that it should first pick up the key to open the door. Fig.~\ref{fig:trajectories} shows two successful and one failed trajectories using our method. Our model learns the two different modes of the desirable behavior. In the fail case, the agent picks up the key but later drops it. Although it still reaches the goal eventually and satisfies the task specifications, it does not finish within the required number of steps.

%  as specified in~\eqref{eq:doorkey_ltl}








==> tex/RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}


% Learning task decompositions and subgoals.
Hierarchical reinforcement learning and options framework \cite{Sutton1999Temporal, Kulkarni2016HRL, Bacon2017Option, Riemer2018Learning} deal with learning task decomposition and temporal extraction. Fox~et~al.~\cite{Fox2017DeepOptions} introduce a multi-level hierarchical model to discover options from demonstrations. Option boundaries are inferred to segment trajectories into different regimes and a control policy is learned for each option.
Kipf~et~al.~\cite{Kipf2019Compile} use an unsupervised encoder-decoder model to predict soft sub-task segmentations and categorial latent encoding for each segment. In this work, we assume tasks can be expressed in LTL formulas and jointly learn it with a cost function to imitate demonstrations. 

% IRL
IRL approaches have been successful in learning behaviors from demonstrations \cite{Neu2012Apprenticeship, Ng2000IRL, Ratliff2006MMP}. Early works assume that the cost is linear in the state features and minimizes the difference in the feature expectation under the learned policy and the feature of the demonstrations. \cite{Ratliff2006MMP} formulates the problem by finding an optimal policy whose expected reward is larger than that of any other policy by a margin. \cite{Ziebart2008MaxEnt} develops a dynamic programming algorithm that finds a maximum entropy policy matching the feature expectation. While IRL methods can perform well in point-to-point navigation tasks, they can struggle in learning temporally-extended and logically-compositional tasks. In this work, we learn such high-level abstractions of the task and use the learned automaton to help learn a cost function of accepting sequences.  

% Learning LTL
LTL is a formal verification language that can express a wide range of logical and temporal task objectives. There are extensive literature in motion planning \cite{Fu2016Optimal, Ding2011MDP,Castro2013Incremental, Sadigh2014ControlSynthesis} and in reinforcement learning \cite{Hasanbeig2019DeepSynth} with the tasks expressed as LTL formulas. In this work, we do not assume that the LTL formula is known and it has to be infered from positive or negative demonstrations. Shah~et~al.~\cite{Shah2018Bayesian} present a probabilistic model for inferring task specification as a temporal logic formula via Bayesian inference. Jeppu~et~al.~\cite{Jeppu2020Learning} develop a program synthesis technique to extract automata, which correspond to LTL formulas. Chou~et~al.~\cite{Chou2020LTL} consider a similar setting to ours and learn the atomic propositions, temporal logic formula and cost parameters in tandem. In particular, they treat the LTL formula as a directed acyclic graph model and learn graph connectivity from demonstrations. Our approach instead relies on a spectral method that learns a WFA equivalent to an LTL formula by correctly classifying accepting and rejecting sequences of symbols. 



